Information-Theoretic Causal Bounds under Unmeasured Confounding

We develop a data-driven information-theoretic framework for sharp partial identification of causal effects under unmeasured confounding. Existing approaches often rely on restrictive assumptions, such as bounded or discrete outcomes; require external inputs (for example, instrumental variables, proxies, or user-specified sensitivity parameters); necessitate full structural causal model specifications; or focus solely on population-level averages while neglecting covariate-conditional effects. We overcome all four limitations simultaneously by establishing novel information-theoretic, data-driven divergence bounds. Our key theoretical contribution shows that the f-divergence between the observational distribution P(Y | A = a, X = x) and the interventional distribution P(Y | do(A = a), X = x) is upper bounded by a function of the propensity score alone. This result enables sharp partial identification of conditional causal effects directly from observational data, without requiring external sensitivity parameters, auxiliary variables, full structural specifications, or outcome boundedness assumptions. For practical implementation, we develop a semiparametric estimator satisfying Neyman orthogonality (Chernozhukov et al., 2018), which ensures root-n consistent inference even when nuisance functions are estimated via flexible machine learning methods. Simulation studies and real-world data applications, implemented in the GitHub repository (https://github.com/yonghanjung/Information-Theretic-Bounds), demonstrate that our framework provides tight and valid causal bounds across a wide range of data-generating processes.

==> settings/commands-ICML.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math notation 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Graphs 
% \newcommand{\CI}{\mathrel{\perp\mspace{-10mu}\perp}}
% \newcommand{\olineo}{\circ\mspace{-7mu}-\mspace{-7mu}\circ}
% \newcommand{\orightarrow}{\circ\!\!\rightarrow}
% \newcommand{\oleftarrow}{\leftarrow\!\!\circ}
% \newcommand{\sleftarrow}{\leftarrow\mspace{-7.5mu}*}
% \newcommand{\srightarrow}{*\mspace{-7.5mu}\rightarrow}
% \newcommand{\slineo}{*\mspace{-6mu}-\mspace{-6mu}\circ}
% \newcommand{\olines}{\circ\mspace{-6mu}-\mspace{-6mu}*}
% \newcommand{\slines}{*\mspace{-6mu}-\mspace{-6mu}*}
% \newcommand{\directedpath}{--\mspace{-5mu}\rightarrow}
% \newcommand{\divergentpath}{\leftarrow \mspace{-5mu} * \mspace{-5mu}\rightarrow}    
% \newcommand{\G}{\mathcal{G}}
% \newcommand{\Gin}[1]{\mathcal{G}_{\overline{#1}}}
% \newcommand{\Gout}[1]{\mathcal{G}_{\underline{#1}}}
% \newcommand{\Gio}[2]{\mathcal{G}_{\overline{#1}\underline{#2}}}


% %%% Notations 
% \newcommand{\omf}[2]{\overline{#1}^{#2}}
% \newcommand{\mf}[1]{\mathbf{#1}}
% \newcommand{\pre}[2]{\text{pre}_{#1}(#2)}
% \newcommand{\prev}[1]{\text{pre}(#1)}
% \newcommand{\ogeq}[2]{\mf{#1}^{\geq #2}}
% \newcommand{\oleq}[1]{\mf{#1}^{i \leq}}
% \newcommand{\lr}[1]{\left(#1\right)}
% \newcommand{\lrp}[1]{\left\{#1\right\}}
% \newcommand{\lrb}[1]{\left[#1\right]}
% \newcommand{\doo}[1]{\operatorname{do}(#1)}

% %%% Math  
% \newcommand{\domain}[1]{\mathfrak{D}_{#1}}
% \newcommand{\support}[1]{\mathfrak{S}_{#1}}
% \newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}
% \newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
% \newcommand{\notimplies}{\mathrel{{\ooalign{\hidewidth$\not\phantom{=}$\hidewidth\cr$\implies$}}}}
% \newcommand{\abs}[1]{\left\vert #1 \right\vert}
% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newcommand{\I}[2]{\mathbb{I}_{#1}(#2)}
% \newcommand{\deriv}[1]{\frac{\partial}{\partial #1}}
% \newcommand{\deriveval}[2]{(\partial / \partial #1)\vert_{#2}}
% \newcommand{\integral}[3]{\int_{#1} #2 \;d[#3]}

% %%% Estimator  
% \newcommand{\mean}[1]{\mathbb{E}[#1]}
% \newcommand{\meani}[2]{\mathbb{E}_{#1}[#2]}
% \newcommand{\variance}[1]{\mathbb{V}[#1]}
% \newcommand{\variancei}[2]{\mathbb{V}_{#1}[#2]}
% \newcommand{\bigmean}[1]{\mathbb{E}\left[#1\right]}
% \newcommand{\bigmeani}[2]{\mathbb{E}_{#1}\left[#2\right]}
% \newcommand{\bigvariance}[1]{\mathbb{V}\left[#1\right]}
% \newcommand{\bigvariancei}[2]{\mathbb{V}_{#1}\left[#2\right]}
% \newcommand{\ith}[2]{#1_{(#2)}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Setting 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\definecolor{opaquegray}{RGB}{192, 192, 192}
\definecolor{afblue}{RGB}{0,0,102}
\definecolor{mypink}{RGB}{255,51,153}

% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{assumption}{Assumption}
% \newtheorem{example}{Example}
% \newtheorem{lemma}{Lemma}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{preliminary}{Preliminary}
% \newtheorem{remark}{Remark}
% \newtheorem{axiom}{Axiom}
% \newtheorem{principle}{Principle}
% \newtheorem{task}{Task}

% Example for Definition
\tcolorboxenvironment{definition}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{theorem}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{corollary}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{lemma}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{proposition}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{proof}{
  colback=white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{example}{
  colback=white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{remark}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{assumption}{
  colback=white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

% % Example for Theorem
% \tcolorboxenvironment{theorem}{
%   colback=red!5!white,
%   colframe=red!80!black,
%   fonttitle=\bfseries,
%   boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
%   % sharp corners,
%   breakable,
% }

% % Example for Lemma
% \tcolorboxenvironment{lemma}{
%   colback=orange!5!white,
%   colframe=orange!80!black,
%   fonttitle=\bfseries,
%   boxrule=0.5pt,
%   % sharp corners,
%   breakable,
% }

% % Example for Example (demonstration)
% \tcolorboxenvironment{example}{
%   colback=green!5!white,
%   colframe=green!80!black,
%   fonttitle=\bfseries,
%   boxrule=0.5pt,
%   % sharp corners,
%   breakable,
% }


==> settings/commands-JMLR.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math notation 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Graphs 
% \newcommand{\CI}{\mathrel{\perp\mspace{-10mu}\perp}}
% \newcommand{\olineo}{\circ\mspace{-7mu}-\mspace{-7mu}\circ}
% \newcommand{\orightarrow}{\circ\!\!\rightarrow}
% \newcommand{\oleftarrow}{\leftarrow\!\!\circ}
% \newcommand{\sleftarrow}{\leftarrow\mspace{-7.5mu}*}
% \newcommand{\srightarrow}{*\mspace{-7.5mu}\rightarrow}
% \newcommand{\slineo}{*\mspace{-6mu}-\mspace{-6mu}\circ}
% \newcommand{\olines}{\circ\mspace{-6mu}-\mspace{-6mu}*}
% \newcommand{\slines}{*\mspace{-6mu}-\mspace{-6mu}*}
% \newcommand{\directedpath}{--\mspace{-5mu}\rightarrow}
% \newcommand{\divergentpath}{\leftarrow \mspace{-5mu} * \mspace{-5mu}\rightarrow}    
% \newcommand{\G}{\mathcal{G}}
% \newcommand{\Gin}[1]{\mathcal{G}_{\overline{#1}}}
% \newcommand{\Gout}[1]{\mathcal{G}_{\underline{#1}}}
% \newcommand{\Gio}[2]{\mathcal{G}_{\overline{#1}\underline{#2}}}


% %%% Notations 
% \newcommand{\omf}[2]{\overline{#1}^{#2}}
% \newcommand{\mf}[1]{\mathbf{#1}}
% \newcommand{\pre}[2]{\text{pre}_{#1}(#2)}
% \newcommand{\prev}[1]{\text{pre}(#1)}
% \newcommand{\ogeq}[2]{\mf{#1}^{\geq #2}}
% \newcommand{\oleq}[1]{\mf{#1}^{i \leq}}
% \newcommand{\lr}[1]{\left(#1\right)}
% \newcommand{\lrp}[1]{\left\{#1\right\}}
% \newcommand{\lrb}[1]{\left[#1\right]}
% \newcommand{\doo}[1]{\operatorname{do}(#1)}

% %%% Math  
% \newcommand{\domain}[1]{\mathfrak{D}_{#1}}
% \newcommand{\support}[1]{\mathfrak{S}_{#1}}
% \newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}
% \newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
% \newcommand{\notimplies}{\mathrel{{\ooalign{\hidewidth$\not\phantom{=}$\hidewidth\cr$\implies$}}}}
% \newcommand{\abs}[1]{\left\vert #1 \right\vert}
% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newcommand{\I}[2]{\mathbb{I}_{#1}(#2)}
% \newcommand{\deriv}[1]{\frac{\partial}{\partial #1}}
% \newcommand{\deriveval}[2]{(\partial / \partial #1)\vert_{#2}}
% \newcommand{\integral}[3]{\int_{#1} #2 \;d[#3]}

% %%% Estimator  
% \newcommand{\mean}[1]{\mathbb{E}[#1]}
% \newcommand{\meani}[2]{\mathbb{E}_{#1}[#2]}
% \newcommand{\variance}[1]{\mathbb{V}[#1]}
% \newcommand{\variancei}[2]{\mathbb{V}_{#1}[#2]}
% \newcommand{\bigmean}[1]{\mathbb{E}\left[#1\right]}
% \newcommand{\bigmeani}[2]{\mathbb{E}_{#1}\left[#2\right]}
% \newcommand{\bigvariance}[1]{\mathbb{V}\left[#1\right]}
% \newcommand{\bigvariancei}[2]{\mathbb{V}_{#1}\left[#2\right]}
% \newcommand{\ith}[2]{#1_{(#2)}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Setting 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\definecolor{opaquegray}{RGB}{192, 192, 192}
\definecolor{afblue}{RGB}{0,0,102}
\definecolor{mypink}{RGB}{255,51,153}

% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
% \newtheorem{example}{Example}
% \newtheorem{lemma}{Lemma}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{preliminary}{Preliminary}
% \newtheorem{remark}{Remark}
% \newtheorem{axiom}{Axiom}
% \newtheorem{principle}{Principle}
% \newtheorem{task}{Task}

% Example for Definition
\tcolorboxenvironment{definition}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{theorem}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{corollary}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{lemma}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{proposition}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{proof}{
  colback=white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{example}{
  colback=white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{remark}{
  colback=gray!5!white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

\tcolorboxenvironment{assumption}{
  colback=white,
  colframe=black,
  % colback=blue!5!white,
  % colframe=blue!80!black,
  fonttitle=\bfseries,
  boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
  breakable,
  % sharp corners,
}

% % Example for Theorem
% \tcolorboxenvironment{theorem}{
%   colback=red!5!white,
%   colframe=red!80!black,
%   fonttitle=\bfseries,
%   boxrule=0.5pt, % Adjust this value for thinner or thicker boundary
%   % sharp corners,
%   breakable,
% }

% % Example for Lemma
% \tcolorboxenvironment{lemma}{
%   colback=orange!5!white,
%   colframe=orange!80!black,
%   fonttitle=\bfseries,
%   boxrule=0.5pt,
%   % sharp corners,
%   breakable,
% }

% % Example for Example (demonstration)
% \tcolorboxenvironment{example}{
%   colback=green!5!white,
%   colframe=green!80!black,
%   fonttitle=\bfseries,
%   boxrule=0.5pt,
%   % sharp corners,
%   breakable,
% }


==> settings/no-circulation-box.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% No Circulate Tag
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \vtop{
     \vspace{-9.5cm}
     \hspace{3cm}
     \begin{tikzpicture}
         % \centering 
         \node [mybox] (box){
           \begin{minipage}[t!]{0.6\textwidth}
             \centering
             Preliminary draft. Please do not circulate or cite. %cite or distribute.
           \end{minipage}
         };
     \end{tikzpicture}
 }
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> settings/package-author-added-ICML.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Added by authors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{wrapfig}
\usepackage{mdframed}
% \usepackage[authoryear,round]{natbib}
\usepackage{tikz}
\usetikzlibrary{positioning,shadows,arrows,shapes,shapes.arrows,arrows.meta,trees,shapes.misc,shapes.geometric,decorations.pathreplacing,calc}
\tikzset{
    -Latex,auto,node distance =1 cm and 1 cm,semithick,
    % state/.style ={ellipse, draw, minimum width = 0.7 cm},
    state/.style ={circle, draw=white, inner sep=0.01cm, minimum width = 0.35 cm},
    snode/.style = {rectangle, draw, inner sep=0.1cm,node contents={}},
    unmeasured/.style = {circle, draw, inner sep=0.05cm,node contents={}},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}
}
\tikzstyle{mybox} = [draw=gray, fill=gray!20, very thick,
rectangle, rounded corners, inner xsep=3pt, inner ysep=7pt]
\usepackage{bm}

\usepackage[on]{settings/editing}
\usepackage{enumerate}
\usepackage{cancel}
\usepackage{multirow}
\usepackage{color}
\usepackage{authblk,epstopdf}
\usepackage{array} % for better arrays (eg matrices) in maths
\usepackage{paralist}
\usepackage{verbatim} % adds environment for commenting out blocks of text & for better verbatim
% \usepackage[noline, ruled, boxed, linesnumbered, vlined]{algorithm2e}
% \usepackage{caption}   % after caption, before algorithm2e
% \usepackage{subcaption}   % after caption, before algorithm2e
\usepackage[normalem]{ulem}
\usepackage{thmtools}
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{lmodern}
\usepackage{setspace}
\usepackage{adjustbox}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage[useregional]{datetime2}
\usepackage{clipboard}
\usepackage{enumitem,kantlipsum} 
\usepackage[some]{background}
\usepackage{optidef}
\usepackage[most]{tcolorbox}
\tcbuselibrary{theorems}
\usepackage{longtable}
\usepackage{ltablex}
\usepackage{nccmath}
% \usepackage{minted} % disabled in CI (requires -shell-escape)
\usepackage{pifont}
\usepackage{sansmath}
% \usepackage{booktabs,tabularx}    % nicely-formatted tables
\usepackage{makecell}  



\definecolor{betterred}{RGB}{228,26,28}
\definecolor{betterblue}{RGB}{55,126,184}

\newcommand\labelAndRemember[2]
  {\expandafter\gdef\csname labeled:#1\endcsname{#2}%
   \label{#1}#2}
\newcommand\recallLabel[1]
   {\csname labeled:#1\endcsname\tag{\ref{#1}}}


\input{settings/commands-ICML}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorlinks=true, citecolor=afblue, linkcolor=RoyalBlue]{hyperref}%


==> settings/package-author-added-JMLR.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Added by authors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{wrapfig}
\usepackage{mdframed}
% \usepackage[authoryear,round]{natbib}
\usepackage{tikz}
\usetikzlibrary{positioning,shadows,arrows,shapes,shapes.arrows,arrows.meta,trees,shapes.misc,shapes.geometric,decorations.pathreplacing,calc}
\tikzset{
    -Latex,auto,node distance =1 cm and 1 cm,semithick,
    % state/.style ={ellipse, draw, minimum width = 0.7 cm},
    state/.style ={circle, draw=white, inner sep=0.01cm, minimum width = 0.35 cm},
    snode/.style = {rectangle, draw, inner sep=0.1cm,node contents={}},
    unmeasured/.style = {circle, draw, inner sep=0.05cm,node contents={}},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}
}
\tikzstyle{mybox} = [draw=gray, fill=gray!20, very thick,
rectangle, rounded corners, inner xsep=3pt, inner ysep=7pt]
\usepackage{bm}

\usepackage[on]{settings/editing}
\usepackage{enumerate}
\usepackage{cancel}
\usepackage{multirow}
\usepackage{color}
\usepackage{authblk,epstopdf}
\usepackage{array} % for better arrays (eg matrices) in maths
\usepackage{paralist}
\usepackage{verbatim} % adds environment for commenting out blocks of text & for better verbatim
% \usepackage[noline, ruled, boxed, linesnumbered, vlined]{algorithm2e}
% \usepackage{caption}   % after caption, before algorithm2e
% \usepackage{subcaption}   % after caption, before algorithm2e
\usepackage[normalem]{ulem}
\usepackage{thmtools}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{lmodern}
\usepackage{setspace}
\usepackage{adjustbox}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage[useregional]{datetime2}
\usepackage{clipboard}
\usepackage{enumitem,kantlipsum} 
\usepackage[some]{background}
\usepackage{optidef}
\usepackage[most]{tcolorbox}
\tcbuselibrary{theorems}
\usepackage{longtable}
\usepackage{ltablex}
\usepackage{nccmath}
% \usepackage{minted} % disabled in CI (requires -shell-escape)
\usepackage{pifont}
\usepackage{sansmath}
\usepackage{booktabs,tabularx}    % nicely-formatted tables
\usepackage{makecell}  
\usepackage{float}



\definecolor{betterred}{RGB}{228,26,28}
\definecolor{betterblue}{RGB}{55,126,184}

\newcommand\labelAndRemember[2]
  {\expandafter\gdef\csname labeled:#1\endcsname{#2}%
   \label{#1}#2}
\newcommand\recallLabel[1]
   {\csname labeled:#1\endcsname\tag{\ref{#1}}}


\input{settings/commands-JMLR}
\usepackage[dvipsnames]{xcolor}
% \usepackage[colorlinks=true, citecolor=afblue, linkcolor=RoyalBlue]{hyperref}%

